An Inner Product on Adelic Measures: With Applications to the Arakelov-Zhang Pairing

We define an inner product on a vector space of adelic measures over a number field. We find that the norm induced by this inner product governs weak convergence at each place of $K$. The canonical adelic measure associated to a rational map is in this vector space, and the square of the norm of the difference of two such adelic measures is the Arakelov-Zhang pairing from arithmetic dynamics. We prove a sharp lower bound on the norm of adelic measures with points of small adelic height. We find that the norm of a canonical adelic measure associated to a rational map is commensurate with the Arakelov height on the space of rational functions with fixed degree. As a consequence, the Arakelov-Zhang pairing of two rational maps $f$ and $g$ can be bounded from below as a function of $g$.

==> adelic_heights.tex <==
\section{Heights and Measures with Small Points}\label{sec: heights and small points}

In this section, we prove a formula relating the adelic height of a probability measure, the Arakelov height, and the norm induced by our inner product. Using this formula, lower bounds on the Arakelov height, and the Arithmetic Equidistribution Theorem (discovered independently in \cite{baker2006equidistribution}, \cite{favre2006equidistribution}, \cite{chambert2006mesures}), we complete the proof of Theorem \ref{thm: lower bounds on norms}.

\subsection{Heights of Adelic Measures}

We summarize some of the discussion in \cite{favre2006equidistribution} and \cite{fili2017metric}. Given an element $\alpha \in \P^1(\bar{K})$ and a place $v\in M_K$,  we denote by $[\alpha]_v$ the probability measure on $\Pberk$ supported equally on the Galois conjugates of $\alpha$ over $K$; thus 

\[ [\alpha]_v = \frac{1}{|\Gal(\bar{K}/K)\cdot \alpha| }\sum_{x \in \Gal(\bar{K}/K)\cdot \alpha} \delta_x.\]

Each $x \in \Gal(\bar{K}/K)\cdot \alpha$ is viewed as an element of $\Pberk$ via an embedding $\bar{K} \hookrightarrow \C_v$; averaging over the Galois conjugates of $\alpha$ ensures that the choice of embedding is irrelevant. We write $[\alpha]$ to denote the adelic probability measure $[\alpha] = ([\alpha]_v)_{v \in M_K}$. Given a proper log-continuous adelic probability measure $\mu = (\mu_v)_{v \in M_K}$, we define 
 \[ \<\mu_v - [\alpha]_v, \mu_v - [\alpha]_v\>_v^* = \iint_{\Pberk \times \Pberk \setminus \Diag_v} \log \frac{1}{||x, y||_v} d(\mu_v - [\alpha]_v)\otimes(\mu_v - [\alpha]_v)(x,y),\]
where $\Diag_v = \{(x, x): x \in \P^1(\C_v)\}$. This is finite by log-continuity of $\mu_v$.  The \textit{height of $\mu$} is the function $h_{\mu}: \P^1(\bar{K}) \to \R$ defined by

\textcolor{red}{THIS MIGHT BE WRONG:} The measure $\mu - [\alpha]$ doesn't assign mass $0$ to $\Aberk\times \Aberk \setminus \Diag$, and so that you can replace the ordinary distance with the chordal distance is not obvious. A better proof: Expand $U_{\mu, v}(x)$ locally, and then average over Galois conjugates and sum over places. You should get $\Ubf_{\mu}(\alpha) = h_\Ar(\alpha) - h_\mu(\alpha)  + h_\mu(\infty) + \Ubf_\mu(\infty)$. Then expand $\frac{1}{2}\|\mu\|^2$ at each place and sum to find that $\|\mu\|^2 = 2h_\mu(\infty) + \Ubf_\mu(\infty)$. 

\begin{equation}\label{eq: height of a measure} h_\mu(\alpha) = \frac{1}{2}\sum_{v \in M_K} r_v \<\mu_v - [\alpha]_v, \mu_v - [\alpha]_v\>^*_v. \end{equation}

A calculation entirely similar to that of remark \ref{rem: mep and inner product} shows that 
\[\<\mu_v - [\alpha]_v, \mu_v - [\alpha]_v\>_v^* = (\!( \mu_v -[\alpha]_v, \mu_v - [\alpha]_v)\!)_v,\] 
and so this agrees with the height of an adelic measure defined in \cite{favre2006equidistribution}. By Theorem 4 of \cite{favre2006equidistribution}, the height of the canonical measure associated to a rational map $f$ agrees with the Call-Silverman canonical height of $f$: $h_{\mu_f}  = h_f$. In particular, as $\lambda_{\std} = \mu_{z^2}$ and $h_{z^2} = h$ (the usual naive height), then $h_{\lambda_{\std}} = h$. \\

Equation \ref{eq: height of a measure} allows us to relate the height of an adelic probability measure to the norm of that measure. We recall that the Arakelov height of $\alpha  \in \P^1(\bar{K})\setminus\{\infty\}$ is given by
\begin{equation}\label{eq: arakelov height def ratio} h_{\Ar}(\alpha) =  \sum_{w \in M_L} r_w \log \frac{1}{||\alpha, \infty||_w}   \end{equation}
where $L/K$ is a finite extension with $\alpha \in \P^1(L)$ and $r_w = [L_w:\Q_w]/[L:\Q]$. We set $h_{\Ar}(\infty) = 0$.  An equivalent definition of the Arakelov height is 

\begin{equation}\label{eq: arakelov height galois} 
h_{\Ar}(\alpha) = \frac{1}{N}\sum_{i = 1}^N \sum_{v \in M_K} r_v \log \frac{1}{||\alpha_i, \infty||_v} 
\end{equation}

where $\alpha_1, ..., \alpha_N$ are the $\Gal(\bar{K}/K)$-conjugates of $\alpha$. Given $\mu \in \Aad$, it is useful to define a function $\Ubf_\mu: \P^1(\bar{K}) \to \C$ by
\[ \Ubf_\mu(\alpha) = \frac{1}{N}\sum_{i = 1}^N \sum_{v \in M_K} r_v U_{\mu, v}(\alpha_i), \]
where $U_{\mu, v}$ are the local potentials of $\mu$. We call $\Ubf_\mu$ the \textit{global potential function associated to $\mu$}. When $\mu = \mu_f$ is the canonical adelic measure associated to a rational map $f$, we will often write $\Ubf_f$ rather than the more cumbersome $\Ubf_{\mu_f}$. With this notation in hand, Equation \ref{eq: height of a measure} can be reformulated as follows.

\begin{prop}\label{prop: pot rep canonical height}
Let $\mu = (\mu_v)_{v \in M_K} \in \Aad$ be an adelic probability measure. For all $\alpha \in \P^1(\bar{K})$ 
\[ h_\mu(\alpha) = h_{\Ar}(\alpha) - \Ubf_\mu(\alpha) + \frac{1}{2}\|\mu\|^2.\]
\end{prop}

\begin{proof}
\textcolor{red}{EDIT 2/12/2023.}\\
Suppose first that $\alpha = \infty$. Then $h_\Ar(\infty) = 0$, and $h_\mu(\infty) = \frac{1}{2}(\!( \mu, \mu)\!)$. Applying the fact that $|x-y|_v ||x, \infty||_v ||y, \infty||_v = ||x, y||_v$ we obtain
\[  \int\int \log \frac{1}{||x,y||_v}\; d\mu_v(x)d\mu_v(y) =  \iint \log\frac{1}{|x-y|_v} \; d\mu_v(x)\;d\mu_v(y) + 2\int \log\frac{1}{||\infty, x||_v}\; d\mu_v(x)    \]
so that 
\[  \|\mu\|_v^2 = (\!(\mu, \mu)\!)_v + 2U_{\mu, v}(\infty).  \]
Multiplying by the ratio of local-to-global degrees and summing over all places of $K$ shows that
\[  \|\mu\|^2 = 2h_\mu(\infty) + 2\Ubf_\mu(\infty).  \]
As $h_\Ar(\infty) = 0$, this implies that $h_\mu(\infty) = -\Ubf_\mu(\infty) + \frac{1}{2}\|\mu\|^2$.\\
Now assume that $\alpha \neq \infty$. Let $\alpha_1, ..., \alpha_n$ be the $\Gal(\bar{K}/K)$ conjugates of $\alpha$. Then
\begin{align*}
   \frac{1}{n}\sum_{i=1}^n U_{\mu, v}(\alpha_i) &= \frac{1}{n}\sum_{i=1}^n \int \log \frac{1}{||\alpha_i, x||_v}\; \mu_v(x) \\
                       &= \frac{1}{n}\sum_{i=1}^n \int \log \frac{1}{|\alpha_i - x|_v||\alpha_i, \infty||_v ||x, \infty||_v}\; \mu_v(x)\\
                       &= (\!(\mu, [\alpha])\!)_v + \frac{1}{n}\sum_{i=1}^n \log \frac{1}{\alpha_i, \infty||_v} + U_{\mu, v}(\infty).
\end{align*}   
Multiplying by the ratio of local-to-global degrees and summing over all places of $K$ then gives
\[   \Ubf_\mu(\alpha) = (\!(\mu, [\alpha])\!) + h_\Ar(\alpha) + \Ubf_\mu(\infty),  \]
where we have applied (\ref{eq: arakelov height galois}). That $\Ubf_\mu(\infty) = \frac{1}{2}\|\mu\|^2 -  \frac{1}{2}h_\mu(\infty)$ implies
\[  (\!(\mu, [\alpha])\!) + \Ubf_\mu(\infty) = \frac{1}{2}\|\mu\|^2 + (\!(\mu, [\alpha])\!) - h_\mu(\infty).   \]
Moreover, $(\!( [\alpha], [\alpha])\!) = 0$ by the product formula and so 
\[  h_\mu(\alpha) = (\!( \mu - [\alpha], \mu - [\alpha])\!) =  h_\mu(\infty) - (\!(\mu, [\alpha])\!). \]
Therefore
\[  (\!(\mu, [\alpha])\!) + \Ubf_\mu(\infty) = \frac{1}{2}\|\mu\|^2 - h_\mu(\alpha),  \]
and it follows that 
\[  \Ubf_\mu(\alpha) = h_\Ar(\alpha) - h_\mu(\alpha) + \frac{1}{2}\|\mu\|^2.  \]
\end{proof}

\begin{rem} We note that as $||\cdot, \cdot||_v$ is valued in $[0,1]$ for all $v$, then $U_{\mu, v}$ is non-negative at each place when $\mu \in \Aad$ is an adelic probability measure. Hence $\Ubf_\mu \geq 0$ on $\P^1(\bar{K})$; it follows at once from Proposition \ref{prop: pot rep canonical height} that $h_\mu(\alpha) - h_\Ar(\alpha) \leq \frac{1}{2}\|\mu\|^2$ for all $\alpha \in \P^1(\bar{K})$. It would be interesting to give a comparable lower bound on $h_\mu - h_\Ar$ in terms of $\|\mu\|^2$. 
\end{rem}

\subsection{A Lower Bound for Adelic Measures with Small Points} 

We say that an adelic probability measure $\mu \in \Aad$ \textit{has small points} or \textit{is a small-point measure} if there is a sequence of distinct points $\{\alpha_n\}_{n=1}^\infty$ in $\P^1(\bar{K})$ with $h_\mu(\alpha_n) \to 0$ as $n \to \infty$. For example, the canonical adelic measure associated to a rational map $f$ always has small points, as $h_f(\alpha) = 0$ for all $\alpha \in \PrePer(f)$. Combining Proposition \ref{prop: pot rep canonical height} with Theorem 2 of \cite{favre2006equidistribution} gives the following relationship between the Arakelov height and the norm of a measure with small points. 

\begin{prop}\label{prop: arakelov height small point norm}
Let $\{\alpha_n\}_{n=1}^\infty$ be a sequence of distinct points in $\P^1(\bar{K})$ with $h_\mu(\alpha_n) \to 0$ as $n \to \infty$. Then $h_\Ar(\alpha_n) \to \frac{1}{2}\|\mu\|^2$ as $n \to \infty. $
\end{prop}

\begin{proof}
Let $\alpha_{n, 1}, ..., \alpha_{n, N}$ be the $\Gal(\bar{K}/K)$-conjugates of $\alpha_n$.  As $U_{\mu, v}$ is continuous at each place, then Theorem 2 of \cite{favre2006equidistribution} implies 
\[ \frac{1}{N}\sum_{i=1}^N U_{\mu, v}(\alpha_{n, i}) \to \int U_{\mu, v}\; d\mu_v = \|\mu_v\|_v^2 \]
as $n \to \infty$. As $U_{\mu, v} = 0$ for all but finitely many $v$, it follows that $\Ubf_\mu(\alpha_n) \to \|\mu\|^2$. So Proposition \ref{prop: pot rep canonical height} implies
 \[0 = \lim_{n \to \infty} h_\mu(\alpha_n) = \lim_{n \to \infty} h_\Ar(\alpha_n) -\frac{1}{2}\|\mu\|^2.\]
\end{proof}

Before completing the proof of Theorem \ref{thm: lower bounds on norms}, we need the following relationships between the Arakelov height and the standard height. 

\begin{lem}\label{lem: arakelov std small points}
Let $\alpha \in \P^1(\bar{K})$. Then 
\begin{enumerate}
    \item  $h_\Ar(\alpha) - \frac{1}{2}\log 2 \leq h(\alpha) \leq h_\Ar(\alpha)$;
    \item $0 \leq h_\Ar(\alpha) - \frac{1}{2}\log 2$ for all $\alpha \neq 0, \infty$;
    \item If $\{\alpha_n\}_{n =1}^\infty$ is a sequence of distinct points in $\P^1(\bar{K})$, then $h_\Ar(\alpha_n) \to \frac{1}{2}\log 2$ if and only if $h(\alpha_n) \to 0$. 
\end{enumerate}
\end{lem}


The proof is elementary albeit rather lengthy. We defer it to the end of this section. We can now complete the proof of Theorem \ref{thm: lower bounds on norms}.

\begin{thm}\label{thm: minimal norm small points}
Let $\mu \in \Aad$ be an adelic probability measure with small points. Then $\|\mu\|^2 \geq \log 2$ with equality if and only if $\mu = \lambda_{\std}$. 
\end{thm}

\begin{proof}
From Lemma \ref{lem: arakelov std small points}, $h_\Ar(\alpha) \geq \frac{1}{2}\log 2$ for all $\alpha \in \P^1(\bar{K}) \setminus \{0 ,\infty\}$. It is then immediate from Proposition \ref{prop: arakelov height small point norm} that $\|\mu\|^2 \geq \log(2)$. To see that this holds exactly when $\mu = \lambda_\std$, we recall Theorem 9 of \cite{fili2017metric}. When combined with Remark \ref{rem: mep and inner product}, this states that if $\{\alpha_n\}_{n=1}^\infty$ is a sequence of distinct points in $\P^1(\bar{K})$ with $h_\mu(\alpha_n) \to 0$, then $h_\nu(\alpha_n) \to \frac{1}{2}\|\mu- \nu\|^2$ for any adelic height $h_\nu$. In particular, if $h_\mu(\alpha_n) \to 0$ then
\begin{equation}\label{eq: weil height to norm} h(\alpha_n) \to \frac{1}{2}\|\mu - \lambda_\std\|^2 \qas n \to \infty. \end{equation}
Combining Lemma \ref{lem: arakelov std small points}, Proposition \ref{prop: arakelov height small point norm}, and (\ref{eq: weil height to norm}) shows that 
\[  \frac{1}{2}\log 2 = \frac{1}{2}\|\mu\|^2 = \lim_{n \to \infty} h_\Ar(\alpha_n) \iff 0 = \frac{1}{2}\|\mu - \lambda_\std\|^2 = \lim_{n \to \infty} h(\alpha_n). \]
\end{proof}

There is a consequence to Proposition \ref{prop: arakelov height small point norm} worth recording here. 
\begin{cor}\label{cor: norm bounds standard measure}
Suppose that $\mu \in \Aad$ is an adelic probability measure with small points. Then $\|\mu\|^2 -\log(2) \leq \|\mu - \lambda_\std\|^2 \leq \|\mu\|^2$.
\end{cor}

\begin{proof}
 Let $\{\alpha_n\}_{n=1}^\infty$ be a sequence of distinct points in $\P^1(\bar{K})$ with $h_\mu(\alpha_n) \to 0$. By Lemma \ref{lem: arakelov std small points}, $h_\Ar(\alpha_n) -\frac{1}{2}\log 2 \leq h(\alpha_n) \leq h_\Ar(\alpha_n)$ for all $n$. Now take the limit as $n \to \infty$ and apply Proposition \ref{prop: arakelov height small point norm} and (\ref{eq: weil height to norm}).
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem: arakelov std small points}.]
Fix a non-zero $\alpha \in \bar{K}$ and let $L$ be a finite extension of $K$ containing $\alpha$. Explicitly, (\ref{eq: arakelov height def ratio}) states that
\[ h_\Ar(\alpha) = \sum_{w \in M_L^\infty} r_w \log \sqrt{1 + |\alpha|_w^2} + \sum_{w \in M_L^0} r_w \log^+ |\alpha|_w.  \]
It is a consequence of the product formula that $h_\Ar(\alpha) = h_\Ar(\alpha^{-1})$ and so, using the fact that $\sum_{w\in M_L^\infty} r_w =1$,

\begin{equation}\label{eq: arakelov height and phi}  4h_\Ar(\alpha) - \log(4) = \sum_{w \in M_L^\infty} r_w \log\frac{(1 + |\alpha|_w^2)(1 + |\alpha|_w^{-2})}{4} + 2\sum_{w\in M_L^0} r_w |\log |\alpha|_w |.\end{equation}

Since $(1 + x^2)(1 + x^{-2})/4 \geq 1$ for all $x\in \R$, it follows that $4h_\Ar(\alpha) \geq \log(4)$. This shows the second item. See also \cite{fili2017energy} for an alternative proof. Writing $h(\alpha)$ as $h(\alpha) = \sum_{w\in M_L} r_w \log^+|\alpha|_w$ and applying the trivial inequalities $\sqrt{1 + |\alpha|_w^2} \geq \max(1, |\alpha|_w) \geq \sqrt{(1 + |\alpha|_w^2)/2}$ at Archimedean places shows the first item of the lemma. For the last claim, let $\{\alpha_n\}_{n=1}^\infty$ be a sequence of distinct points in $\P^1(\bar{K})$. 
By the first and second items of the lemma, if $h(\alpha_n) \to 0$ then 
\[  0 = \lim_{n \to \infty} h(\alpha_n) \geq \lim_{n \to \infty} h_{\Ar}(\alpha_n) - \frac{1}{2}\log 2 \geq 0.  \]
Hence $\lim_{n \to \infty} h_\Ar(\alpha_n) = \frac{1}{2}\log 2$. The converse is more delicate. \\

We are going to show that there is an absolute constant $A > 1$ so that 

\begin{equation}\label{eq: arakelov height minus log 2}
     2h_\Ar(\alpha) - \log(2) +  \sqrt{A( h_\Ar(\alpha) - \frac{1}{2}\log 2)} \geq h(\alpha).
\end{equation}  

for all $\alpha \in \P^1(\bar{K})\setminus\{0, \infty\}$. From this it follows that $h_\Ar(\alpha_n) \to \frac{1}{2}\log 2$ implies $h(\alpha_n) \to 0$. 
We prove (\ref{eq: arakelov height minus log 2}) by studying the two real-valued functions $\phi, \psi: (0, \infty) \to [0, \infty)$ defined by 
\[  \phi(x) =  \log \frac{(1 + x^2)(1 + x^{-2})}{4}\; \; \text{and}\;\; \psi(x) = |\log x|. \]
Note that if $x > 1$, then $\phi(x) - \psi(x) \geq 0$ if and only if $(1 + x^2)(1 + x^{-2}) - 4x \geq 0$. This is true precisely when $x \geq \theta$, where $\theta \approx 3.38298$ is the unique real root of the polynomial $x^3 - 3x^2 - x - 1$. Note that $\phi(\theta) = \psi(\theta)$. That both $\phi$ and $\psi$ are invariant under the change of variables $x \mapsto x^{-1}$ shows that $\phi(x) - \psi(x) \geq 0$ when $x < \theta^{-1}$. Thus $\phi(x) \geq \psi(x)$ for all $x \in (0, \infty)\setminus [\theta^{-1}, \theta]$. Now the function $\psi^2/\phi$ is continuous on $[\theta^{-1}, \theta]\setminus \{1\}$, and, an application of l'Hopital's rule shows that $\lim_{x \to 1} \psi^2(x)/\phi(x) = 1$. Thus $\psi^2/\phi$ is bounded above on $[\theta^{-1}, \theta]$. It is not hard to see that this bound is achieved at the endpoints. Consequently $\psi^2(x)/\phi(x) \leq \psi^2(\theta)/\phi(\theta) = \psi(\theta) = \log \theta \approx 1.21876$ for all $x \in [\theta^{-1}, \theta]$. \\

Let $I = [\theta^{-1}, \theta]$ and let $\chi_I$ be the indicator function of $I$. Set $A = \log \theta$. It follows from the above considerations that if $x_1,..., x_N$ is a sequence of positive real numbers then 
\[ \frac{A}{N}\sum_{i=1}^N \phi(x_i) \geq \frac{1}{N}\sum_{i=1}^N \chi_I(x_i) \psi^2(x_i). \] %\geq \left( \frac{1}{N}\sum_{i=1}^N \chi_I(x_i) \psi(x_i)\right)^2, \]
Applying Jensen's inequality to the average $(1/N)\sum_{i=1}^N \chi_I^2(x_i) \psi^2(x_i)$ shows
\[ \frac{1}{N}\sum_{i=1}^N \chi_I(x_i) \psi^2(x_i) \geq \left( \frac{1}{N}\sum_{i=1}^N \chi_I(x_i) \psi(x_i)\right)^2,  \]
where we have used the fact that $\chi_I^2 = \chi_I$. Therefore
\begin{equation}\label{eq: bound in bad interval}
    \left( \frac{A}{N}\sum_{i=1}^N \phi(x_i) \right)^{1/2} \geq \frac{1}{N}\sum_{i=1}^N \chi_I(x_i) \psi(x_i).
\end{equation}

That $\phi(x) \geq \psi(x)$ for all $x \notin I$ implies

\begin{equation}\label{eq: bound off of bad interval}
    \frac{1}{N}\sum_{i=1}^N \phi(x_i) \geq \frac{1}{N}\sum_{i=1}^N (1 - \chi_I(x_i))\psi(x_i).
\end{equation}

Finally, consider the sequence of positive numbers $\{ |\alpha|_w\}_{w \in M_L^\infty}$, where each $|\alpha|_w$ is repeated with multiplicity $[L_w : \R]$. Counting multiplicities there are $[L: \Q]$ such numbers, so applying (\ref{eq: bound in bad interval}) and (\ref{eq: bound off of bad interval}) to this sequence shows

\[ \sum_{w \in M_L^\infty} r_w \phi(|\alpha|_w) +  \left( A\sum_{w \in M_L^\infty} r_w \phi(|\alpha|_w) \right)^{1/2} \geq \sum_{w \in M_L^\infty} r_w \psi(|\alpha|_w).  \]

This inequality and (\ref{eq: arakelov height and phi}) imply
\begin{align*}
    4h_\Ar(\alpha) - \log(4) + (A( 4h_\Ar(\alpha) - \log(4)))^{1/2} &\geq 4h_\Ar(\alpha) - \log(4) +   \left( A\sum_{w \in M_L^\infty} r_w \phi(|\alpha|_w) \right)^{1/2} \\
                                                                    &= \sum_{w \in M_L^\infty} r_w \phi(|\alpha|_w)  + 2\sum_{w \in M_L^0}r_w \psi(|\alpha|_w) +\\
                                                                    &\;\;+ \left( A\sum_{w \in M_L^\infty} r_w \phi(|\alpha|_w) \right)^{1/2}\\
                                                                    &\geq \sum_{w \in M_L^\infty} r_w |\log|\alpha|_w| + 2\sum_{w \in M_L^0} r_w |\log|\alpha|_w|\\
                                                                    &\geq \sum_{w \in M_L} r_w |\log |\alpha|_w |\\
                                                                    &= 2h(\alpha).
\end{align*}
Dividing this final inequality by $2$  gives (\ref{eq: arakelov height minus log 2}). 
\end{proof}

There is a corollary to this proof which provides an upper bound on the norm of the difference between $\lambda_\std$ and  a measure with small points. 

\begin{cor}\label{cor: convergence to log 2 gives congergence of az pairing}
    Suppose that $\mu = (\mu_v)_{v\in M_K}$ is an adelic probability measure with points of small height. Then  there is an absolute constant $A>1$ so that 
    \[  \|\mu\|^2 - \log(2) +  \sqrt{A( \frac{1}{2}\|\mu\|^2 - \frac{1}{2}\log 2)} \geq \frac{1}{2}\|\mu - \lambda_\std\|^2.   \]
\end{cor}

\begin{proof}
    Let $(\alpha_n)_{n=1}^\infty$ be a sequence with $h_\mu(\alpha_n) \to 0$. Then, from \ref{eq: arakelov height minus log 2}, take the limit of
    \[ 2h_\Ar(\alpha_n) - \log(2) +  \sqrt{A( h_\Ar(\alpha_n) - \frac{1}{2}\log 2)} \geq h(\alpha_n)\]
    as $n \to \infty$ and use the fact that $h_\Ar(\alpha_n) \to \frac{1}{2}\|\mu\|^2$ and $h(\alpha_n) \to \frac{1}{2}\|\mu - \lambda_\std\|^2$. 
\end{proof}

==> small_point_proof.tex <==
We end this section by proving the statements in Remark \ref{rem: small points intro} from the introduction. What follows summarizes some of the discussion in \cite{favre2006equidistribution} and \cite{fili2017metric}. Given an element $\alpha \in \P^1(\bar{K})$ and a place $v\in M_K$,  we denote by $[\alpha]_v$ the probability measure on $\Pberk$ supported equally on the Galois conjugates of $\alpha$ over $K$; thus 

\[ [\alpha]_v = \frac{1}{|\Gal(\bar{K}/K)\cdot \alpha| }\sum_{x \in \Gal(\bar{K}/K)\cdot \alpha} \delta_x.\]

Each $x \in \Gal(\bar{K}/K)\cdot \alpha$ is viewed as an element of $\Pberk$ via an embedding $\bar{K} \hookrightarrow \C_v$; averaging over the Galois conjugates of $\alpha$ ensures that the choice of embedding is irrelevant. We write $[\alpha] = ([\alpha]_v)_{v \in M_K}$. 

Recall that $\mu$ \textit{has points of small height} if there is a sequence $\{\alpha_n\}_{n=1}^\infty$ of distinct points in $\P^1(\bar{K})$ so that
\[ h_{\mu}(\alpha_n) \to 0 \;\;\text{as}\;\; n \to \infty, \]
where
\[ h_{\mu}(\alpha) := \frac{1}{2} (\!( \mu - [\alpha], \mu - [\alpha])\!) \]
is the Favre--Rivera-Letelier height associated to $\mu$. The \textit{Arakelov height} of a point $\alpha = [a:b] \in \P^1(\bar{K})$ is defined to be 
\[ h_{\Ar}(\alpha) = \sum_{v \in M_L^\infty} r_v \log \sqrt{|a|_v^2 + |b|_v^2} + \sum_{v \in M_K^0} r_v \log\max( |a|_v, |b|_v),  \]
where $L/K$ is finite extension containing $\alpha$. 

\begin{prop}\label{prop: small points}
Let $\mu$ be an adelic probability measure and $\{\alpha_n\}_{n=1}^\infty$ a sequence in $\P^1(\bar{K})$ with $h_\mu(\alpha_n) \to 0$. Then $h_\Ar(\alpha_n) \to \frac{1}{2}\|\mu\|^2$ as $n \to \infty$. Moreover $\|\mu\|^2 \geq \log(2)$ with equality if and only if $\mu = \lambda_\std$. 
\end{prop}

\begin{proof}
    We observe that 
    \[ (\!( \lambda_\Ar, \lambda_\Ar)\!) = \frac{-1}{2}, \;\; (\!( \alpha, \lambda_\Ar)\!) = h_{\Ar}(\alpha), \;\; \text{and}\;\; (\!([\alpha], [\alpha])\!) = 0.\]
    The first equality is a consequence of \ref{prop: arakelov jensen}, the second follows from \ref{prop: arakelov jensen} and the definition of the Arakelov height, and the third is by the product formula. It follows that $h_{\lambda_\Ar}(\alpha) = -1/4 + h_{\Ar}(\alpha)$ for all $\alpha\in \P^1(\bar{K})$. \\
    Suppose that $\{\alpha_n\}_{n=1}^\infty$ is a sequence of distinct points in $\P^1(\bar{K})$ so that $h_{\mu}(\alpha_n) \to 0$. Then $h_{\lambda_\Ar}(\alpha_n) \to \frac{1}{2}\|\mu- \lambda_\Ar\|^2 = \frac{1}{2}\|\mu\|^2 - \frac{1}{4}$. So $h_{\Ar}(\alpha_n) \to \frac{1}{2}\|\mu\|^2$ as $n \to \infty$. \\
    Now $h_\Ar(\alpha) \geq \frac{1}{2}\log(2)$ for all $\alpha \in \P^1(\bar{K}) \setminus\{0, \infty\}$ \cite{fili2017energy}. Therefore $\frac{1}{2}\|\mu\|^2 = \lim_{n \to \infty} h_{\Ar}(\alpha_n) \geq \frac{1}{2}\log(2)$. A straightforward computation shows that $\|\lambda_\std\|^2= \frac{1}{2}\log(2)$; see Proposition \ref{prop: norm of conjugation of squaring map} for a more general statement. Lastly, if $\|\mu\|^2 = \log(2)$ then $h_{\Ar}(\alpha_n) \to \frac{1}{2}\log(2)$. It is known that this implies $[\alpha_n]_v \to \lambda_{\std, v}$ weakly at each place of $K$; see, for instance, Example 6.5 of \cite{gil2019distribution}. On the other hand, $[\alpha_n]_v$ converges weakly to $\mu_v$ at each place and so $\mu = \lambda_\std$. 
\end{proof}
